Pronoun Logic

Particularly in transgender and nonbinary (TGNB) communities, it is an increasingly common practice to publicly share one's personal pronouns so that we may be gendered correctly in others' speech. Many of us have nuanced desires for how we are gendered, leading us to use more complex descriptions of our wishes; for example, the descriptor 'she/they'. We observe that these descriptions of our wishes have the structure of a little language all their own. We thus propose formal logic as a tool for expressing one's personal pronouns and potentially other aspects of gender. We explore three potential logical foundations (linear logic, temporal logic, and free logic with definite descriptions) and their trade-offs. Our foremost motivation for this proposal is play, affirming that one can be both a logician and TGNB at the same time. We present formalization as something that can continue to evolve over time with society's understanding of gender. This implies that outreach is a major potential application: we can show TGNB youth that they belong in logic and have a unique contribution to make. Tools for evaluating whether one's pronouns are respected are an application as well.

==> meeting-notes-and-todo.tex <==
*** 2/2/2024
Tentative venue: Queer in AI 2024.
March 30th
https://www.queerinai.com/naacl-2024

Neth's interests:
- Has an interest in making a dating app
- We choose to reveal ourselves to different people different amounts
- Might not want to share them on an app for privacy
- Pronouns can change over time
- e.g. "only queer people can call me it/its"
   - comes in both private and public versions

TODO List for Neth for this week:
1) Switch the paper over to ACL format. Queer in AI call has a link to the relevant files
2) Epistemic logic, especially dynamic epistemic logic.
   Epistemic logic is the logic of what you know.
   (related: doxastic logic, belief)
   Start reading from: 
     https://plato.stanford.edu/entries/logic-epistemic/
   Follow references as time allows.
   If you need something but have no access, ask Rose
3) Come prepared to talk about how epistemic logic might be used in modeling pronouns

TODO List for Rose:
- Come prepared to walk through paper structure

==> review-info.tex <==
is lolli broken

free logci presentation hard

Mathy

implication

